A bounded-noise mechanism for differential privacy

We present an asymptotically optimal $(\epsilon,\delta)$ differentially private mechanism for answering multiple, adaptively asked, $\Delta$-sensitive queries, settling the conjecture of Steinke and Ullman [2020]. Our algorithm has a significant advantage that it adds independent bounded noise to each query, thus providing an absolute error bound. Additionally, we apply our algorithm in adaptive data analysis, obtaining an improved guarantee for answering multiple queries regarding some underlying distribution using a finite sample. Numerical computations show that the bounded-noise mechanism outperforms the Gaussian mechanism in many standard settings.

==> adaptive-data-analysis.tex <==
\section{Application to adaptive data analysis}

Adaptive data analysis is a setting where an analyst would like to compute multiple adaptively-chosen queries on some underlying distribution $P$, while having access only to a finite i.i.d. sample  $X_1 \cdots X_n \sim P$. The simplest setting concerns statistical queries, where each query $i$ is given by some function $q_i$ from the underlying domain to $[-1,1]$, and the goal is to approximate $\E_{X\sim P}[q_i(X)]$. The simplest approach is to output as an answer the sample-average $a_i = \frac{1}{n}\sum_{j=1}^n[q_i(X_j)]$. This is valid if the $q_i$ are independent of the data. However, here each $q_i$ can be chosen adversarially given the previous answers $a_1,\dots,a_{i-1}$.  which depend on the data, hence they can be selected to fool this simple algorithm. In order to avoid this issue, CITE suggested to answer the queries with differential privacy, thus avoiding the possibility that the queries are tailored against the specific dataset. They provide the following condition for an algorithm to be $(\alpha,\beta)$ accurate, namely, to satisfy $\max_i |a_i - \E_{X\sim P}[q_i(X)]| \le \alpha$ w.pr. $1-\beta$:
\begin{theorem}[CITE]
Fix parameters $\alpha,\beta \in (0,1/2)$. Assume that the answers $a_1,\dots,a_n$ to $q_1,\dots,q_k$ satisfy the following:
\begin{itemize}
\item The answers $(\alpha,\alpha\beta)$ differential privacy with respect to the dataset $(X_1,\dots,X_n)$.
\item The answers are $(\alpha,\alpha\beta)$ accurate with respect to the \emph{sample}:
$
\max_{i\in \{1,\dots,k\}} \lp| a_i - \frac{1}{n}\sum_{j=1}^n q_i(X_j) \rp| \le \alpha
$
w.pr. $1-\alpha\beta$.
\end{itemize}
Then, the answers are $(O(\alpha),O(\beta))$-accurate w.r.t. $P$: $\max_i |a_i - \E_{X\sim P}[q_i(X)]| \le O(\alpha)$ w.pr. $1-O(\beta)$.
\end{theorem}

As a consequence, one obtains the following sample bounds on differentially private question-answering strategies (which are the best known at the moment):
\begin{corollary}[CITE]
The Gaussian mechanism and the sparse vector mechanism of CITE are $(\alpha,\beta)$ accurate w.rt. $P$ with sample complexities of
\[
n \le O\lp(\frac{\sqrt{k \log k \log^2(1/\alpha\beta)}}{\alpha^2}\rp), \quad \text{and }
n \le O\lp(\frac{\sqrt{k \log\log k \log^3(1/\alpha\beta)}}{\alpha^2}\rp), \quad \text{(respectively).}
\]
\end{corollary}
Applying the bounded-noise mechanism, we obtain the following result:
\begin{corollary}
For any $\alpha,\beta \in (0,1/2)$ s.t. $\alpha\beta \ge e^{-k/\log^8 k}$, the bounded-noise mechanism with parameters $\epsilon = O(\alpha)$ and $\delta = O(\alpha\beta)$ is $(\alpha,\beta)$-accurate, with sample complexity
\[
n \le O\lp(\frac{\sqrt{k \log(1/\alpha\beta)}}{\alpha^2}\rp).
\]
Further, the dependence on $k$ and $\beta$ is tight (CITE).
\end{corollary}
Since BNM has both an improved dependence on $k$ and its noise is bounded w.pr. $1$, we obtain a bound that improves both the dependence on $k$ and on $\log(1/\alpha\beta)$. The most significant improvement is on the failure probability $\beta$: a small failure probability is necessary if adaptive data analysis is part of a complex algorithm many ingredients, each having a small failure probability.

==> older-general.tex <==
\section{Older}

Here is the formal statement of the problem: \begin{question}
    Find a distribution $\mu$ over $\mathbb{R}^d$ that satisfies the following:
    \begin{itemize}
        \item $\E_{x\sim \mu}[\|x\|_\infty] \le O(1)$.
        \item For any $v \in \mathbb{R}^d$ with $\|v\|_\infty \le 1/\sqrt{d}$,
        \[
        \E_{x\sim \mu}|\log\mu(x) - \log \mu(x+v)| \le O(1).
        \]
    \end{itemize}
\end{question}

Notice that if we take $\mu(x) \propto e^{-d\|x\|_K}$ for some convex set $K$, then the distribution is roughly uniform over the surface of $K$. We can we-write the question as follows:
\begin{question}\label{q:conv-sets}
    Find a convex set $K$ that satisfies the following:
    \begin{itemize}
        \item 
            $\E_{x\sim \partial K}[\|x\|_\infty] \le O(1)$,
            where $x\sim \partial K$ means that $x$ is uniform from the surface of $K$.
        \item 
            For any $v\in\mathbb{R}^d$ that satisfies $\|v\|_\infty \le 1/\sqrt{d}$, 
            \[
            \E_{x\sim \partial K}\lp|1 - \|x+v\|_K\rp| \le O(1/d).
            \]
    \end{itemize}
\end{question}

We give two examples for sets $K$:
\begin{example}[The cube.]
    Consider $K = \{x \colon \|x\|_\infty \le 1\}$. Then, the first requirement trivially holds. The second requirement does not, becasue a perturbation of $v$ modifies the infinity by an order approximately $1/\sqrt{d}$.
\end{example}

\begin{example}
    Consider  $K = \sqrt{d} B_2 = \{x \colon \|x\|_2 \le \sqrt{d}\}$. Then, the first requirement is off by a $\sqrt{\log d}$ factor. The second requirement, however, holds. Indeed, fix any $v$ with $\|v\|_\infty \le 1/\sqrt{d}$ and notice that for a random $x \sim \partial K$,
    \[
    \|x + v\|_K = \|x+v\|_2/\sqrt{d}.
    \]
    Noting that $v$ is small compared to $x$, we have that
    \[
    |1 - \|x+v\|_K| \approx |1-\|x+v\|_K^2|
    = |1 - \|x+v\|_2^2/d|
    = |1 - \|x\|_2^2/d - x^\top v/d -\|v\|_2^2/d|.
    \]
    Since $\|x\|_2 = \sqrt{d}$, and $\|v\|_2 \le \sqrt{d}\|v\|_\infty \le 1$, we have
    \[
    |1 - \|x\|_2^2/d - x^\top v/d -\|v\|_2^2/d|
    = |x^\top v/d +\|v\|_2^2/d|
    \le |x^\top v/d| + 1/d.
    \]
    Our goal is to bound the last quantity by $O(1/d)$. Since $x$ is drawn uniformly from $\sqrt{d}B_2$, we have that
    \[
    \E[|x^\top v/d|]
    \le O(\|v\|_2/d)
    \le O(1/d)
    \]
    as required.
\end{example}

\paragraph{Local behavior of Minkowski's norm}
Let us make a first-order approximation of the norm $\|x+v\|_K$ at some point $x$. We can write $\|x+v\|_K \approx (x+v)^\top g(x)$ for a small $v$ and some vector $g(x)$. Notice that $n(x):= g(x)/\|g(x)\|_2$ is the normal to $K$ at the point $x$ and that $1=\|x\|_K=x^\top g(x)$. Hence, we derive that
\[
g(x) = \frac{n(x)}{|x^\top n(x)|}.
\]
Re-writing condition 2, we want to bound by $O(1/d)$ the following quantity:
\[
\E_{x\sim \partial K} |1 - \|x+v\|_K|
\approx \E_{x\sim \partial K}
\lp|1 - (x+v)^\top g(x) \rp|
= \E |v^\top g(x)|
= \E \lp|\frac{v^\top n(x)}{x^\top n(x)} \rp|.
\]
Notice that it is likely to have $|v^\top n(x)| \le O(1/\sqrt{d})$ since $\|v\|_2\le 1,\|n(x)\|_2=1$ and also, $n(x)$ is roughly uniform. Hence, our goal is roughly to show that $\E 1/|x^\top n(x)| \le O(1/\sqrt{d})$.
In other words, we want to say that
\[
|x^\top n(x)| \ge c\sqrt{d}
\]
typically.
Hence, we derive the following question:
\begin{question}[informal]\label{q:first-approx}
Find a convex set $K$ that satisfies:
\begin{itemize}
    \item $\E_{x\sim \partial K} \|x\|_\infty \le O(1)$.
    \item For a typical value of $x\in \partial K$, $x^\top n(x) \ge \Omega(\sqrt{d})$.
\end{itemize}
\end{question}
Let's look at the examples above. In the first example, $K = B_\infty$, for any $x\in \partial K$ we have that $n(x) = (0,\dots,0,1,0,\dots,0)$, namely, one value of $1$ in the maximal entry of $x$. Hence, $x^\top n(x) = 1$. And in the second example $K = \sqrt{d}B_2$, we have that $n(x) = x/\|x\|_2$. Hence $x^\top n(x) = \|x\|_2 = \sqrt{d}$ as required.

\paragraph{A stupid attempt that may work.}
We look at the original question. And we want to have $\mu(x) \propto \exp(-\sum_i f(x_i))$ where $f(x)$ is some function. We want $f(x)$ to be defined only on $[-1,1]$ such that $\lim_{x\to 1} f(x) = \infty$, and say, $f(-x) = f(x)$. Further, notice that $\sum_i f(x_i+v_i) - \sum_i f(x_i) = \sum_i f'(x_i)v_i + f''(\xi_i) v_i^2$ where $\xi_i$ is a point in the line between $x_i$ and $x_i+v_i$. We want $f'(x_i)$ to be $O(1)$ with fast decaying tails and also something similar for $f''(\xi_i)$.

For example, take $f(x) = (1-|x|)^{-2}$. Notice that $|f'(x)| \approx (1-|x|)^{-3}$. To bound the Orlics norm of the first derivative, calculate
\[
\E e^{ c |f'(x)|^{2/3}}
= \int e^{ c (1-|x|)^{-2} - (1-|x|)^{-2}}
\le O(1).
\]
Now, we also need the second derivative to be bounded appropriately. We have $f''(x) = C(1-|x|)^{-4}$. As long as $x \le 1-2/\sqrt{d}$, we have that $f''(\xi_i)$ is of the same order as $f''(x_i)$. Hence, our goal is twofold:
\begin{itemize}
    \item 
        Show concentration of $f''(x_i)$
    \item Bound the probability that $x_i     \ge 1-2/\sqrt{d}$.
\end{itemize}
The probability for too-large $x$ is bounded by $e^{-C d}$. For the second requirement, we have $f''(x) = (1-|x|)^{-4}$. So, we have that
\[
\E e^{c |f''(x)|^{1/2}} \le O(1).
\]

We might need to take instead $C(1-x^2)^{-p}$ for some sufficiently large $p>0$ and this will get what we want for all $\delta \ge 1/k$. For a smaller $\delta$, we might want to modify the function to enable the random variable to get larger. This will ensure that the derivatives cannot get too large.

% \paragraph{An improvement over the previous attempt}
% Notice that if we take instead $f(x) = (1-|x|)^{-p}$ where $p$ is a large constant, we improve our guarantees! Because now the convergence is even better. The only place we are losing is in the approximation of $\xi_i$ by $x_i$: the larger the approximation is, the worse is the bound. So, we should select it appropriately to get an appropriate bound.

% We might need to find a different function $f$ for each $d$. That's because the union bound that we do over the $d$ coordinates. On the other hand, this might be okay, because in the summation over $d$ terms, the subGaussian tail gets larger as $d$ gets larger. So, we need to make sure that the random variables are decaying in a fast enough pace up to the point that the subExponential does not dominate any more, and then move to a subGaussian setting.

==> older-proof.tex <==
\newpage

To apply Lemma~\ref{lem:Taylor} on $\ADER{R}$, we would like to analyze the derivatives of $\fDER{R}$. Since $\fDER{R}(\eta) = \fDE(\eta/R)$, it suffices to analyze the derivatives of $\fDE$. First, we bound the deviations of single instances of $\fDE'(\eta)$ and $\fDE''(\eta)$ and later analyze sums of independent instances. (The proof appears in Section~\ref{sec:pr:properties})
\begin{restatable}{lemma}{lemSingleConcentrate}
	\label{lem:singleConcentrate}
	For any $t \ge 2$, $\Pr[|\fDE'(\eta)| > t] \le C\exp(-ct/\log^2 t)$ and $\Pr[|\fDE''(\eta)| > t] \le C\exp(-c t/\log^4 t)$ where $c,C>0$ are universal constant.
\end{restatable}

Next, we would like to analyze concentration for sums of independent instances of $\fDE'(\eta_i)$ and $\fDE''(\eta_i)$. For that purpose, we use a general result on concentration of sums of independent random variables, which follows from \cite{bakhshizadeh2020sharp}. (The proof appears in Section~\ref{sec:pr:sums})

\begin{restatable}{lemma}{lemSumsMain}\label{lem:sums-main}
	Let $X$ be a random variable with $\Pr[|X|>t] \le \exp(-I(t))$ for all $t > 0$, for some monotonic non-decreasing function $I(t)$. Assume that $ t^{\gamma}/C \le I(t) \le Ct$ for some $C,\gamma>0$ and all $t > 0$. Let $X_1,\dots,X_k$ be i.i.d. copies of $X$. Then, there exists $c > 0$ that depends only on the law (i.e. distribution) of $X$, such that for all $t > 0$,
	\[
	\Pr\lp[\lp|\sum_i X_i -  \sum_i \E X_i \rp| > t\rp]
	\le 
	2\exp\lp(-c\min(I(t),t^2/k)\rp) \enspace.
	\]
\end{restatable}

Applying Lemma~\ref{lem:singleConcentrate} and Lemma~\ref{lem:sums-main}, we can get deviation bounds for sums of derivatives of $\fDE$: (The proof appears in Section~\ref{sec:pr:sums})
\begin{restatable}{lemma}{lemSumsFDE}
	\label{lem:dist-main-properties}
	Let $\eta_1,\dots,\eta_k$ be independent copies from $\muDE$ and let $v_1,\dots,v_k \in [-1,1]$. There are universal constants $c,C>0$ such that the following holds:
	\begin{enumerate}
		\item
		For any $t> 0$:
		\[
		\Pr\lp[\lp|\sum_{i=1}^k \fDE'(\eta_i)v_i\rp| > t\rp]
		\le
		2\exp\lp(-c\min\lp(t^2/k,t/\log^2(t)\rp)\rp)\enspace.
		\]
		\item
		For any $t> 0$:
		\[
		\Pr\lp[\sum_{i=1}^k \fDE''(\eta_i) > Ck + t\rp]
		\le \exp\lp(-c\min\lp(t^2/k,t/\log^4(t)\rp)\rp)\enspace.
		\]
	\end{enumerate}
\end{restatable}

Notice that claim 2 of Lemma~\ref{lem:dist-main-properties} does not quite suffice for condition 2 of Lemma~\ref{lem:Taylor}. While Lemma~\ref{lem:dist-main-properties} provides a bound on $\sum_i \fDE''(\eta_i)$, Lemma~\ref{lem:Taylor} requires a bound on $\sum_i \fDE''(\xi_i)$ for some $\xi_i$ in the neighborhood of each $\eta_i$. Hence, we would like to show that with high probability, $\fDE''(\xi_i)$ can be bounded in terms of $\fDE''(\eta_i)$. (The proof appears in Section~\ref{sec:pr:properties}.)
\begin{restatable}{lemma}{lemPerturbation}
	\label{lem:perturbation}
	There exist universal constants $C,C_0>1$ such that for any $u \in (0,1)$,
	\[
	\Pr_{\eta\sim \muDE}\lp[ 
	\sup_{\xi \in [\eta-u,\eta+u]} \fDE''(\xi)
	\le C_0 \fDE''(\eta_i)
	\rp]
	\ge 1-C \exp(-\exp(1/\sqrt{6u}))
	\enspace.
	\]
\end{restatable}

Using the general Lemma~\ref{lem:Taylor} and the analysis of $\fDE$ in Lemma~\ref{lem:dist-main-properties} and Lemma~\ref{lem:perturbation}, we can conclude the proof.
\begin{proof}[Proof of Theorem~\ref{thm:main}]
	We would like to use Lemma~\ref{lem:Taylor}, substituting $f$ with $\fDER{R}$, while Lemma~\ref{lem:dist-main-properties} and Lemma~\ref{lem:perturbation} will be used to show concentration of the first and second derivatives of $\fDER{R}$.
	
	Recall from Definition~\ref{def:DE} that the density of $\muDER{R}$ at $\eta \in (-R,R)$ equals
	\[
	\frac{e^{-\fDER{R}(\eta)}}{\ZDER{R}}, \quad \text{where } \fDER{R}(\eta) = \fDE(\eta/R) \text{ and } \ZDER{R} = R\ZDE.
	\]
	In particular, $\fDER{R}'(\eta) = \fDE'(\eta/R)/R$ and $\fDER{R}''(\eta) = \fDE''(\eta/R)/R^2$. From Lemma~\ref{lem:dist-main-properties} we have that for all $t \ge 0$ and all $v_1,\dots,v_k \in [-1,1]$,
	\begin{align}
	&\Pr_{\eta_1,\dots,\eta_k \simiid \muDER{R}}\lp[\lp|\sum_i v_i \fDER{R}'(\eta_i)\rp| > \epsilon/2 \rp]
	= \Pr_{\eta_1,\dots,\eta_k \sim \mu_{\DE,R}}\lp[\lp|\sum_i v_i \fDE'(\eta_i/R)\rp| > \epsilon R/2 \rp]\notag\\
	&\quad= \Pr_{\eta_1,\dots,\eta_k \sim \mu_{\DE}}\lp[\lp|\sum_i v_i  \fDE'(\eta_i)\rp| > \epsilon R/2 \rp]
	\le 2\exp\lp(-c\min\lp(\epsilon^2 R^2/k,\epsilon R/\log^2(\epsilon R)\rp)\rp)
	\le \delta/3, \label{eq:41}
	\end{align}
	assuming that the constant $C$ in the definition of $R$ is sufficiently large and using the fact that $\delta \ge \exp(-k/\log^8 k)$.
	Similarly, we can bound the sum of second derivatives. Let $C_0>0$ be the constant from Lemma~\ref{lem:perturbation}. Then, Lemma~\ref{lem:dist-main-properties} implies that
	\begin{align}\label{eq:bnd-second}
	&\Pr_{\eta_1,\dots,\eta_k \sim \mu_{\DE,R}}\lp[\sum_i \fDER{R}''(\eta_i) > \epsilon/(2C_0) \rp]
	= \Pr_{\eta_1,\dots,\eta_k \sim \mu_{\DE,R}}\lp[\sum_i \fDE''(\eta_i/R) > \epsilon R^2/(2C_0) \rp]\\
	&= \Pr_{\eta_1,\dots,\eta_k \sim \mu_{\DE}}\lp[\sum_i \fDE''(\eta_i) > \epsilon R^2/(2C_0) \rp]
	\le 2\exp\lp(-c\min\lp(\epsilon^2 R^2/k,\epsilon R/\log^4(\epsilon R)\rp)\rp)
	\le \delta/3.
	\end{align}
	Lastly, recall from Lemma~\ref{lem:Taylor} that instead of bounding $\fDER{R}''(\eta_i)$, we have to bound $\fDER{R}''(\xi_i)$ for some $\xi_i \in [\eta_i-1,\eta_i+1]$. One can bound $\fDER{R}''(\xi_i)$ in terms of $\fDER{R}''(\eta_i)$, using Lemma~\ref{lem:perturbation}:
	\begin{align*}
	&\Pr_{\eta \sim \mu_{\DE,R}}[\exists \xi \in [\eta-1,\eta+1] \text{ s.t. } \fDER{R}''(\xi) > C_0\fDER{R}''(\eta)]\\
	&= \Pr_{\eta\sim \mu_{\DE,R}}[\exists \xi \in [\eta-1,\eta+1] \text{ s.t. } \fDE''(\xi/R) > C_0\fDE''(\eta/R)]\\
	&= \Pr_{\eta'\sim \mu_{\DE}}[\exists \xi' \in [\eta'-1/R,\eta'+1/R] \text{ s.t. } \fDE''(\xi') > C_0\fDE''(\eta')]\\
	&\le C'\exp(-\exp(\sqrt{R/6}))
	\le C'\exp(-\exp(\sqrt{C/6}k^{1/4}))
	\le \exp(-k)/(3k)
	\le \delta/(3k)
	\end{align*}
	where $C'>0$ is a universal constant, $C>0$ is the constant in the definition of $R$ and we assume that $C$ is sufficiently large. By a union bound over $i \in [k]$, one has that
	\[
	\Pr_{\eta_1,\dots,\eta_k\sim \mu_{\DE,R}}[\exists i \in [k], \exists \xi_i \in [\eta_i-1,\eta_i+1] \text{ s.t. } \fDER{R}''(\xi_i) > C_0\fDER{R}''(\eta_i)]
	\le \delta/3.
	\]
	In combination with \eqref{eq:bnd-second},
	\begin{equation} \label{eq:2nd-bnd}
	\Pr_{\eta_1,\dots,\eta_k \sim \mu_{\DE,R}}\lp[\sum_i \max_{\xi_i \in [\eta_i-1,\eta_i+1]}\fDER{R}''(\eta_i) > \epsilon/2 \rp]
	\le 2\delta/3.
	\end{equation}
	\eqref{eq:41} and \eqref{eq:2nd-bnd} suffice to satisfy the requirements of Lemma~\ref{lem:Taylor}, and this concludes that the algorithm is $(\epsilon,\delta)$ differentially private, as required..
\end{proof}


\subsection{Proofs for the general lemmas on $(\epsilon,\delta)$-privacy} \label{sec:pr:general}

\subsection{Properties of the bounded-support distribution}
\label{sec:pr:properties}

Below, we analyze properties of the distribution $\muDE$ and prove Lemma~\ref{lem:singleConcentrate} and Lemma~\ref{lem:perturbation}. For convenience, we denote $f=\fDE$.
%First of all, we estimate the normalizing constant $Z$:
%\begin{lemma}\label{lem:bnd-Z}
%	It holds that
%	\[
%	0.01 \le Z \le 2
%	\]
%\end{lemma}
%\begin{proof}
%	.
%\end{proof}
First, a direct calculation proves the following:
\begin{lemma}\label{lem:bnd-derivatives}
For any $\eta \in (-1,1)$,
\[
f'(\eta) = 2e^{1/(1-\eta^2)}\eta(1-\eta^2)^{-2};\quad 
f''(\eta)
= 2 e^{1/(1-\eta^2)}(1+4\eta^2-3\eta^4)(1-\eta^2)^{-4}
\le 10 e^{1/(1-\eta^2)}(1-\eta^2)^{-4}.
\]
Therefore,
\[
|f'(\eta)| \le 2 f(\eta) \log^2 f(\eta); \quad
0 \le f''(\eta) \le 10 f(\eta) \log^4 f(\eta).
\]
\end{lemma}

Next, we re-state and prove Lemma~\ref{lem:singleConcentrate}.
\lemSingleConcentrate*
\begin{proof}
	For any $\eta$ such that $f'(\eta) \ge t$, it holds from Lemma~\ref{lem:bnd-derivatives} that $t \le f'(\eta) \le 2 f(\eta) \log^2 f(\eta)$. This implies that $f(\eta) \ge c t/\log^2 t$ for some universal constant $c>0$. Hence,
	\begin{align*}
	\Pr_{\muDE}[|f'(\eta)| \ge t]
	&= \frac{1}{\ZDE}\int_{\eta \colon |f'(\eta)|\ge t} \exp(-f(\eta)) d\eta
	\le \frac{1}{\ZDE}\int_{\eta \colon |f'(\eta)|\ge t} \exp(-c t/\log^2 t) d\eta\\
	&\le \frac{1}{\ZDE}\int_{\eta \in [-1,1]} \exp(-c t/\log^2 t) d\eta
	= \frac{2}{\ZDE} \exp(-c t/\log^2 t).
	\end{align*}
	This suffices for the bound on the first derivative since $\ZDE$ is a universal constant.
	The bound with respect to the second derivative follows a similar argument.
\end{proof}

Before proving Lemma~\ref{lem:perturbation}, we present an auxiliary lemma:
\begin{lemma}\label{lem:bnd-sec}
	Let $u \in (0,1/6)$ and let $\eta$ be any number such that $\eta^2 \le 1-\sqrt{6u}$. Then,
	\[
	\max_{\xi\in [\eta-u,\eta+u]} f''(\xi)
	\le 240 f''(\eta).
	\]
\end{lemma}
\begin{proof}
	Since $f''(\eta) = f''(-\eta)$, we can assume that $\eta \ge 0$. Let $\xi \in [\eta-u,\eta+u]$. 
%	Notice that
%	\begin{equation}\label{eq:sec1}
%	1-\eta^2 \ge 1-\eta \ge \sqrt{6u} = \max(\sqrt{6u},6u),
%	\end{equation}
%	using the fact that $|\eta|\le 1$ and $0 \le 6u\le 1$.
	Notice that
	\begin{equation} \label{eq:sec2}
	1 - \xi^2
	\ge 1-(\eta+u)^2
	= 1 - \eta^2 - 2\eta u - u^2
	\ge 1 - \eta^2 - 3u.
	\end{equation}
	By the assumptions of this lemma,
	\[
	3u = \frac{6u}{2} \le \frac{\sqrt{6u}}{2}
	\le \frac{1-\eta^2}{2}.
	\]
	In combination with \eqref{eq:sec2}, one derives
	\begin{equation} \label{eq:sec3}
	1-\xi^2 \ge (1 - \eta^2)/2.
	\end{equation}
	Further, we have from the assumptions of this lemma and from \eqref{eq:sec2} and \eqref{eq:sec3} that
	\begin{equation}\label{eq:sec4}
	\frac{1}{1-\xi^2}
	- \frac{1}{1-\eta^2}
	= \frac{(1-\eta^2)- (1-\xi^2)}{(1-\eta^2)(1-\xi^2)}
	\le \frac{3u}{(1-\eta^2)(1-\xi^2)}
	\le \frac{6u}{(1-\eta^2)^2}
	\le 1\enspace.
	\end{equation}
	From the formula for $f''$ in Lemma~\ref{lem:bnd-derivatives} and from \eqref{eq:sec3} and \eqref{eq:sec4}, one derives that
	\begin{equation}\label{eq:sec5}
	f''(\xi)
	\le 10 e^{1/(1-\xi^2)}(1-\xi^2)^{-4}
	\le 10 e^{1/(1-\eta^2)+1}\frac{16}{(1-\eta^2)^{4}}
	= 160 e \cdot e^{1/(1-\eta^2)} (1-\eta^2)^{-4}.
	\end{equation}
	Lastly, notice from the formula for $f''$ in Lemma~\ref{lem:bnd-derivatives}, from \eqref{eq:sec5} and from $e\le 3$, that
	\[
	f''(\eta)
	\ge 2 e^{1/(1-\eta^2)} (1-\eta^2)^{-4}
	\ge \frac{2}{160e} f''(\xi)
	\ge \frac{1}{240} f''(\xi).
	\]
\end{proof}

%\begin{lemma}
%	Let $\eta_1,\dots,\eta_k$ be independent copies from $\muDE$. There are universal constants $c,C,C_0>0$ such that the following holds:
%	For any $u \in (0,1)$ it holds with probability at least $1-C k \exp(-\exp(\sqrt{6u}))$ that for all $i$, $-1<\eta_i-u < \eta_i+u <1$ and that
%	\[
%	\sup_{\xi \in [\eta_i-u,\eta_i+u]} f''(\xi)
%	\le C_0 f''(\eta_i).
%	\]
%\end{lemma}
We restate and prove Lemma~\ref{lem:perturbation}, using Lemma~\ref{lem:bnd-sec}:
\lemPerturbation*
\begin{proof}
	Using Lemma~\ref{lem:bnd-sec}, it suffices to bound the probability that $\eta^2 > 1-\sqrt{6u}$. 
	For any such $\eta$ one has
	\[
	f(\eta) = \exp(1/(1-\eta^2)) \ge \exp(1/\sqrt{6u}).
	\]
	Hence
	\begin{align*}
	\Pr[\eta^2 > 1-\sqrt{6u}]
	&= \frac{1}{\ZDE} \int_{\substack{\eta\in (-1,1) \colon \\\eta^2 >1-\sqrt{6u}}}
	\exp(-f(\eta)) d\eta
	\le \frac{1}{\ZDE} \int_{\substack{\eta\in (-1,1) \colon \\\eta^2 >1-\sqrt{6u}}}
	\exp(-\exp(1/\sqrt{6u})) d\eta\\
%	
%	
	&\le \frac{1}{\ZDE} \int_{-1}^1
	\exp(-\exp(1/\sqrt{6u})) d\eta
	= \frac{2}{\ZDE}\exp(-\exp(1/\sqrt{6u})).
	\end{align*}
\end{proof}



\subsection{Sums of heavy tailed random variables}
\label{sec:pr:sums}

In this section, we prove Lemma~\ref{lem:sums-main} and Lemma~\ref{lem:dist-main-properties}.
We use the following theorem from \cite{bakhshizadeh2020sharp}:
\begin{theorem}[\cite{bakhshizadeh2020sharp}, Theorem~1 and Remark~1, special case]\label{thm:concentration-prior}
	Suppose $X_1, ..., X_k \overset{d}{=} X$ are independent and identically distributed random variables that satisfy $\Pr[X_i > t]\le \exp(-I(t))$ for some continuous increasing function $I: \mathbb{R} \rightarrow \mathbb{R}^{\geq 0}$ with the property $I(t) = O(t)$ as $t \rightarrow \infty$.   Define $Z^L \triangleq X \mathds{I}(X\le L)- \E X$. Further, for $L>0$ and $\lambda = \frac{I(L)}{2L}$, define
	\begin{align}
	c_{L} \triangleq \E\lp[(Z^L)^2 \mathds{I} \intoo{Z^L \leq 0} + \intoo{Z^L}^2 \expp{\lambda \intoo{Z^L}} \mathds{I} \intoo{Z^L > 0}\rp]
	\end{align}
	and let $\alpha \in \mathbb{R}$ be any number such that $\alpha \ge c_L$ for all $L > 0$.
	Finally, define $t_{\max}(k) \triangleq \sup \lp\{t \geq 0: \; t \leq \frac{\alpha k}{2}  \frac{I(t)}{t} \rp\}$.\footnote{We set $t_{\max}=0$, when the set is empty. } Then,
	\begin{equation} \label{eq:concentration ineq}
	\Pr\lp[\sum_i X_i - \sum_i \E X_i > t\rp]\leq \begin{cases}
	\expp{-I(t)/4} + k \expp{-I(t)} & 
	t \geq t_{\max}(k)
	\\
	\expp{-\frac{t^2}{2 k\alpha} } + k \expp{-  \frac{ 2t_{\max}(k)^2}{\alpha k} } &
	0 \leq t < t_{\max}(k)
	\end{cases} \enspace.
	\end{equation}
\end{theorem}

We re-state and prove Lemma~\ref{lem:sums-main} using Theorem~\ref{thm:concentration-prior}.

\lemSumsMain*
\begin{proof}
We note that throughout the proof, all the constants may depend on the law of $X$. We will bound the right tail of $\sum_i X_i$ and the left tail is bounded similarly.
Using the same argument as Lemma~3(a) from \cite{bakhshizadeh2020sharp}, one has $\lim_{L\to\infty} c_L = \mathrm{Var}(X)$. Further, it follows from definition that $c_L$ is bounded in any bounded subset of $(0,\infty)$ and that $c_L$ is a continuous function of $L$, hence, $c_L$ is uniformly bounded in $(0,\infty)$ by some constant $\alpha >0$.
Applying Theorem~\ref{thm:concentration-prior}, one has
\begin{align}\label{eq:42}
\Pr\lp[\sum_i X_i - \sum_i \E X_i > t\rp]
\le \begin{cases}
\expp{-I(t)/4} + k \expp{-I(t)} & 
t \geq t_{\max}(k)
\\
\expp{-\frac{t^2}{2 k\alpha} } + k \expp{-  \frac{ 2t_{\max}(k)^2}{\alpha k} } &
0 \leq t < t_{\max}(k)
\end{cases}
%\le \begin{cases}
%k \expp{-I(t)/4} & 
%t \geq t_{\max}(\beta)
%\\
%k\expp{-\frac{t^2}{2 k\alpha} } &
%0 \leq t < t_{\max}(\beta)
%\end{cases}\\
%\le k \exp(-\min(t^2/(2 k\alpha), I(t)/4))
%= k \exp(-\min(t^2/(2 k\alpha) - \log k, I(t)/4 - \log k)).
\end{align}
Notice that from the condition that $I(t) \ge t^{\gamma}/C$ for some $C>0$, it follows that \begin{equation}\label{eq:50}
t_{\max}(k) \ge c'' k^{1/(2-\gamma)}
\end{equation}
for some $c''>0$. To bound \eqref{eq:42}, we divide into cases according to $t$. 
\begin{itemize}
	\item If $t \ge t_{\max}(k)$: since $I(t) \ge t^\gamma/C$ and from \eqref{eq:50}, we have that $k\exp(-I(t)) \le C' \exp(-I(t)/4)$ for some $C'>0$. Hence, the right hand side of \eqref{eq:42} is bounded by 
	$(C'+1)\exp(-I(t)/4)$.
	\item If $t \le t_{\max}(k)$: \eqref{eq:50} implies that $t_{\max}^2/k \ge \Omega(k^{2/(2-\gamma)-1})= \Omega(k^{\gamma/(2-\gamma)})$. This implies that $k\exp(-\frac{t_{\max}(k)^2}{\alpha k}) \le C' \exp(-c t_{\max}^2/k) \le C' \exp(-ct^2/k)$ for some $C',c>0$. Hence, the right hand side of \eqref{eq:42} is bounded by $O(\exp(-ct^2/k))$, as required.
\end{itemize}
\end{proof}

We restate and prove Lemma~\ref{lem:dist-main-properties}:
\lemSumsFDE*
\begin{proof}
	For the first item, we apply Lemma~\ref{lem:sums-main} with $X_i = \fDE'(\eta_i)v_i$. %to bound the deviation of $\lp|\sum_i \fDE'(\eta_i)v_i - \E\lp[\sum_i \fDE'(\eta_i)v_i\rp]\rp|$.
	Lemma~\ref{lem:singleConcentrate} implies that we can substitute $I(t) = ct/\log^2 t$, obtaining
	\[
	\Pr\lp[\lp|\sum_{i=1}^k \fDE'(\eta_i)v_i - \sum_{i=1}^k \E\lp[\fDE'(\eta_i)v_i\rp]\rp| > t\rp]
	\le
	2\exp\lp(-c\min\lp(t^2/k,t/\log^2(t)\rp)\rp)\enspace.
	\]
	Further, $\E \fDE'(\eta_i)=0$ for all $i$ due to the following reasons: (1) the function $\fDE'(\eta)$ is antisymmetric, namely, $\fDE'(-\eta)=-\fDE(\eta)$, and (2) distribution $\muDE$ is symmetric around zero. This derives the first claim.
	
	To prove the second claim, we apply Lemma~\ref{lem:sums-main} with $X_i = \fDE''(\eta_i)$. From Lemma~\ref{lem:singleConcentrate} we can substitute $I(t) = ct/\log^4 t$, which derives that
	\[
	\Pr\lp[\sum_{i=1}^k \fDE''(\eta_i) - \sum_{i=1}^k \E \fDE''(\eta_i) > t\rp]
	\le \exp\lp(-c\min\lp(t^2/k,t/\log^4(t)\rp)\rp)\enspace.
	\]
	Further, it follows from Lemma~\ref{lem:singleConcentrate} that $\E \fDE''(\eta_i) < \infty$, hence $\E\lp[\sum_{i=1}^k \fDE''(\eta_i)\rp] \le Ck$ for some constant $C>0$. This concludes the second claim.
\end{proof}

